Adversarial Attacks and Defences Competition

To accelerate research on adversarial examples and robustness of machine learning classifiers, Google Brain organized a NIPS 2017 competition that encouraged researchers to develop new methods to generate adversarial examples as well as to develop new ways to defend against them. In this chapter, we describe the structure and organization of the competition and the solutions developed by several of the top-placing teams.

==> submission_defense_1_tsail_orig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Subsection about submission XXXXXXXX
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{1st place in defense track: team TsAIL}
\label{sec:adv_comp:def1}

\runinhead{Team members:} Yinpeng Dong, Fangzhou Liao, Ming Liang, Tianyu Pang, Jun Zhu and Xiaolin Hu.

In this section, we introduce the High-level representation guided denoiser~(HGD) method, which won the first place in the defense track.
The idea is to train a neural network based denoiser to remove the adversarial perturbation.

%We described how to build a dataset in Sec. \ref{sec:hgd:dataset}, detail the idea in Sec. \ref{sec:hgd:method}, and show some general experiments \ref{sec:hgd:results}, then we show the detail of our submission in Sec. \ref{sec:hgd:submit}.
 
 
\subsubsection{Dataset} \label{sec:hgd:dataset}
To prepare the training set for the denoiser, we first extracted 20K images from the ImageNet training set (20 images per class).
Then we used a bunch of adversarial attacks to distort these images and form a training set.
Attacking methods included FGSM and I-FGSM and were applied to the many models and their ensembles to simulate weak and strong attacks.

\subsubsection{Denoising U-net}
Denoising autoencoder (DAE) \cite{vincent2008extracting} is a potential choice of the denoising network. 
But DAE has a bottleneck for the transmission of fine-scale information between the encoder and decoder.
This bottleneck structure may not be capable of carrying the multi-scale information contained in the images.
That's why we used a denoising U-net (DUNET). 

\begin{figure*}
\includegraphics[width=\linewidth]{figures/tsail/detail_daunet3}
\caption{
The detail of DUNET. The numbers inside each cube stand for width $\times$ height, and the number outside the cube stands for the number of channels. In all the C3 of the feedforward path, the stride of the first C is $2\times2$.}
\label{fig_daunet}
\end{figure*}

Compared with DAE, the DUNET adds some lateral connections from encoder layers to their corresponding decoder layers of the same resolution (Figure \ref{fig_daunet}). 
In this way, the network is learning to predict adversarial noise only ($d\hat{x}$ in Figure \ref{fig_daunet}), which is more relevant to denoising and easier than reconstructing the whole image \cite{zhang2017beyond}. The clean image can be readily obtained by subtracting the noise (adding -$d\hat{x}$) from the corrupted input.


\subsubsection{Loss function} \label{sec:hgd:method}

\begin{figure}
\centering
\includegraphics[width=0.6\columnwidth]{figures/tsail/hgd}
\caption{Diagrams of various denoisers. Upper-left: the vanilla denoiser. Upper-right: feature guided denoiser. Lower-left: the logits guided denoiser. Lower-right: the class-label guided denoiser.}
\label{fig:hgd}
\end{figure}

The vanilla denoiser uses the reconstructing distance as the loss function, but we found a better method.
Given a target neural network, we extract its representation at $l$-th layer for $x$ and $\hat{x}$, and calculate the loss function as:
\begin{equation}
L=|f_l(\hat{x}) - f_l(x)|.
\end{equation}
The corresponding models are called HGD, because the supervised signal comes from certain high-level layers of the classifier and carries guidance information related to image classification. 

We propose two HGDs with different choices of $l$. For the first HGD, we define $l=-2$ as the index of the topmost convolutional layer. This denoiser is called feature guided denoiser (FGD). For the second HGD, we use the logits layer. So it is called logits guided denoiser (LGD). 

Another kind of HGD uses the classification loss of the target model as the denoising loss function, which is supervised learning as ground truth labels are needed. This model is called class label guided denoiser (CGD) (see Fig. \ref{fig:hgd}). Please refer to our full-length paper \cite{liao2017defense} for more information.


